FlexNeRF: Photorealistic Free-viewpoint Rendering of Moving Humans from Sparse Views

We present FlexNeRF, a method for photorealistic freeviewpoint rendering of humans in motion from monocular videos. Our approach works well with sparse views, which is a challenging scenario when the subject is exhibiting fast/complex motions. We propose a novel approach which jointly optimizes a canonical time and pose configuration, with a pose-dependent motion field and pose-independent temporal deformations complementing each other. Thanks to our novel temporal and cyclic consistency constraints along with additional losses on intermediate representation such as segmentation, our approach provides high quality outputs as the observed views become sparser. We empirically demonstrate that our method significantly outperforms the state-of-the-art on public benchmark datasets as well as a self-captured fashion dataset. The project page is available at: https://flex-nerf.github.io/

==> new_ablations.tex <==
% 
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{@{}lcr@{}}
\toprule
Ablation & PSNR $\uparrow$ & $\Delta$ \hspace{1mm} \\
\midrule
HumanNeRF & 26.12 & 0.00 \\ 
Ours (Full) & \textbf{29.55} & \textbf{+3.43} \\ 
Ours (w/o PID) & 27.42 & +1.30 \\
Ours (w/o CO-MLP + CCL) & 28.50 & +2.38 \\
Ours (w/o PID + CO-MLP + CCL) & 26.95 & +0.83 \\
\bottomrule
\end{tabular}
\vspace{-0.12in}
\caption{Ablation on SCF dataset.}
\label{tab:rebuttal_ablation}
\end{table}


% \definecolor{amber}{rgb}{1.0, 0.75, 0.0}
% \begin{table*}[b!]
% \clearpage
% \begin{center}
% \begin{tabular}{ |c|c|c|c| } 
% \hline

% \textbf{Ablation} & \textbf{{LPIPS} $\times \mathbf{10^3}$ $\downarrow$} & \textbf{{PSNR} $\uparrow$} & \textbf{{SSIM} $\uparrow$}\\ 
% \hline
% HumanNeRF & 39.71 & 26.12 & 0.9366 \\ 
% \hline
% HumanNeRF w/ \textcolor{red}{(refinement MLPs + binary segm. loss)} & 38.92 & 26.95 & 0.9412 \\
% \hline
% Ours (full) & \textbf{34.26} & \textbf{29.55} & \textbf{0.9627}\\ 
% \hline
% Ours w/o \textcolor{amber}{pose-indep. temporal deform. MLP} & (37.11) & (27.42) & (0.9469)\\
% \hline
% Ours w/o \textcolor{green}{(can. to obs. MLP + cyc. cons. loss)} & 36.86 & 28.50 & 0.9509 \\ 
% \hline
% Ours w/o \textcolor{magenta}{temp. cons. loss} & 36.17 & 27.94 & 0.9521 \\
% \hline
% % w/o binary segm. & 35.78 & 29.07 & 0.9601 \\
% % \hline
% Ours w/o \textcolor{red}{(refinement MLPs + binary segm. loss)} & 35.91 & 29.02 & 0.9588 \\
% \hline
% \end{tabular}

% \end{center}
% \vspace{-4mm}
%   \caption{Ablation: Effect of removing various modules and losses from our full approach on the SCF dataset.}
%   \label{tab:ablation}
% \end{table*}




==> results_tab_mocap.tex <==
% \begin{table*}[t]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
% \hline
% \multirow{2}{4em}{{Method}} & \multicolumn{3}{|c|}{{Subject 377}} & \multicolumn{3}{|c|}{{Subject 392}} \\
% \cline{2-7}
%  & {LPIPS} $\times \mathbf{10^3}$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$ & {LPIPS} $\times \mathbf{10^3}$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$\\ 
% \hline
% Neural Body \cite{Peng2021NeuralBI} & 40.95 & 29.11 & 0.9674 & 53.27 & 30.10 & 0.9642 \\ 
% \hline
% HumanNeRF \cite{Weng2022HumanNeRFFR} & 24.06 & \textbf{30.41} & 0.9743 & 32.12 & 31.04 & 0.9705 \\ 
% \hline
% Ours & \textbf{23.58} & 30.39 & \textbf{0.9761} & \textbf{30.96} & \textbf{32.17} & \textbf{0.9769}\\ 
% \hline
% \end{tabular}
% \end{center}
% %---------------------------------------------------------------------------
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
% \hline
% \multirow{2}{4em}{{Method}} & \multicolumn{3}{|c|}{{Subject 386}} & \multicolumn{3}{|c|}{{Subject 393}} \\
% \cline{2-7}
%  & {LPIPS} $\times \mathbf{10^3}$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$ & {LPIPS} $\times \mathbf{10^3}$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$\\ 
% \hline
% Neural Body \cite{Peng2021NeuralBI} & 46.43 & 30.54 & 0.9678 & 59.05 & 28.61 &	0.959 \\ 
% \hline
% HumanNeRF \cite{Weng2022HumanNeRFFR} & 28.99 & 33.20 & 0.9752 & 36.72 & 28.31 & 0.9603 \\ 
% \hline
% Ours & \textbf{27.29} & \textbf{34.59} & \textbf{0.9803} & \textbf{33.85} & \textbf{29.87} & \textbf{0.9711}\\ 
% \hline
% \end{tabular}
% \end{center}
% % \cellcolor{blue!10}
% %---------------------------------------------------------------------------
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
% \hline
% \multirow{2}{4em}{{Method}} & \multicolumn{3}{|c|}{{Subject 387}} & \multicolumn{3}{|c|}{{Subject 394}} \\
% \cline{2-7}
%  & {LPIPS} $\times \mathbf{10^3}$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$ & {LPIPS} $\times \mathbf{10^3}$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$\\ 
% \hline
% Neural Body \cite{Peng2021NeuralBI} & 59.47 & 27.00 & 0.9518 & 54.55 & 29.1 & 0.9593 \\ 
% \hline
% HumanNeRF \cite{Weng2022HumanNeRFFR} & 35.58 & 28.18 & 0.9632 & 32.89 & 30.31 & 0.9642 \\ 
% \hline
% Ours & \textbf{32.49} & \textbf{29.57} & \textbf{0.9786} & \textbf{30.76} & \textbf{31.97} & \textbf{0.9709}\\ 
% \hline
% \end{tabular}

% \end{center}
%   \caption{Comparison of various performance metrics on the ZJU-MoCap dataset.}
%   \label{tab:mocap}
% \end{table*}

% %------------------------------------------------------------------------

% \begin{table*}[t]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
% \hline
% \multirow{2}{4em}{{Method}} & \multicolumn{3}{|c|}{{Subject 377}} & \multicolumn{3}{|c|}{{Subject 392}} \\
% \cline{2-7}
%  & {LPIPS} $\times 10^3$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$ & {LPIPS} $\times 10^3$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$\\ 
% \hline
% Neural Body \cite{Peng2021NeuralBI} & 40.95 & 29.11 & 0.9674 & 53.27 & 30.10 & 0.9642 \\ 
% \hline
% HumanNeRF \cite{Weng2022HumanNeRFFR} & 24.06 & \textbf{30.41} & 0.9743 & 32.12 & 31.04 & 0.9705 \\ 
% \hline
% Ours & \textbf{23.58} & 30.39 & \textbf{0.9761} & \textbf{30.96} & \textbf{32.17} & \textbf{0.9769}\\ 
% \hline
% \end{tabular}
% \end{center}
% %---------------------------------------------------------------------------
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
% \hline
% \multirow{2}{4em}{{Method}} & \multicolumn{3}{|c|}{{Subject 386}} & \multicolumn{3}{|c|}{{Subject 393}} \\
% \cline{2-7}
%  & {LPIPS} $\times 10^3$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$ & {LPIPS} $\times 10^3$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$\\ 
% \hline
% Neural Body \cite{Peng2021NeuralBI} & 46.43 & 30.54 & 0.9678 & 59.05 & 28.61 &	0.959 \\ 
% \hline
% HumanNeRF \cite{Weng2022HumanNeRFFR} & 28.99 & 33.20 & 0.9752 & 36.72 & 28.31 & 0.9603 \\ 
% \hline
% Ours & \textbf{27.29} & \textbf{34.59} & \textbf{0.9803} & \textbf{33.85} & \textbf{29.87} & \textbf{0.9711}\\ 
% \hline
% \end{tabular}
% \end{center}
% % \cellcolor{blue!10}
% %---------------------------------------------------------------------------
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c| } 
% \hline
% \multirow{2}{4em}{{Method}} & \multicolumn{3}{|c|}{{Subject 387}} & \multicolumn{3}{|c|}{{Subject 394}} \\
% \cline{2-7}
%  & {LPIPS} $\times 10^3$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$ & {LPIPS} $\times 10^3$ $\downarrow$ & {PSNR} $\uparrow$ & {SSIM} $\uparrow$\\ 
% \hline
% Neural Body \cite{Peng2021NeuralBI} & 59.47 & 27.00 & 0.9518 & 54.55 & 29.1 & 0.9593 \\ 
% \hline
% HumanNeRF \cite{Weng2022HumanNeRFFR} & 35.58 & 28.18 & 0.9632 & 32.89 & 30.31 & 0.9642 \\ 
% \hline
% Ours & \textbf{32.49} & \textbf{29.57} & \textbf{0.9786} & \textbf{30.76} & \textbf{31.97} & \textbf{0.9709}\\ 
% \hline
% \end{tabular}

% \end{center}
%   \caption{Comparison of various performance metrics on the ZJU-MoCap dataset.}
%   \label{tab:mocap}
% \end{table*}
